Adaptation of Agentic AI: A Survey of Post-Training, Memory, and Skills

Large language model (LLM) agents are moving beyond prompting alone. ChatGPT marked the rise of general-purpose LLM assistants, DeepSeek showed that on-policy reinforcement learning with verifiable rewards can improve reasoning and tool use, and OpenClaw highlights a newer direction in which agents accumulate persistent memory and reusable skills. Yet the research landscape remains fragmented across post-training, retrieval, memory, and skill systems. This survey studies these developments under a single notion of \emph{adaptation}: improving an agent, its tools, or their interaction after pretraining. We organize the field with a four-paradigm framework spanning agent adaptation and tool adaptation. On the agent side, A1 (tool-execution-signaled) and A2 (agent-output-signaled) improve the agent itself through supervised fine-tuning, preference optimization, and reinforcement learning with verifiable rewards. On the tool side, T1 (agent-agnostic) provides reusable pre-trained modules any agent can call, while T2 (agent-supervised) uses the agent's outputs to train memory systems, skill libraries, or lightweight subagents. Using this framework, we review post-training methods, adaptive memory architectures, and agent skills; compare their trade-offs in cost, flexibility, and generalization; and summarize evaluation practices across deep research, software development, computer use, and drug discovery. We conclude by outlining open problems in agent-tool co-adaptation, continual learning, safety, and efficient deployment.

==> tables/a1_methods.tex <==
% --- Your original color definitions ---
\definecolor{sectionblue}{RGB}{230,245,255}
\definecolor{sectiongreen}{RGB}{235,255,235}
\definecolor{cardinal}{RGB}{180,0,0}

% --- NEW: Color for the table header ---
\definecolor{white}{RGB}{255,255,255}

% Stylish longtable
\small
%
% == CHANGED HERE ==
% Use \rowcolors* (with asterisk) to reset counter after manual \rowcolor
% Start at row 1, so the first data row after a section header is gray
%
\rowcolors*{1}{gray!7}{white}
\renewcommand{\arraystretch}{1.15}

\begin{longtable}[t]{>{\raggedright\arraybackslash}p{1.2cm}
                  >{\raggedright\arraybackslash}p{2.0cm}
                  >{\raggedright\arraybackslash}p{1.5cm}
                  >{\raggedright\arraybackslash}p{2.4cm}
                  >{\raggedright\arraybackslash}p{2.5cm}
                  >{\raggedright\arraybackslash}p{2.5cm}
                  >{\raggedright\arraybackslash}p{1.8cm}
                  >{\raggedright\arraybackslash}p{0.8cm}}
\rowcolor{white}
\caption{A1 Methods (Tool Execution Signaled): Earlier Methods (SFT \& DPO) and Recent RLVR-based Methods} \\

\toprule
% == CHANGED HERE ==
% Added a background color to the header row
\rowcolor{white}
\textbf{Time} & \textbf{Method} & \textbf{Venue} & \textbf{Task(s)} & \textbf{Tool(s)} & \textbf{Agent Backbone} & \textbf{Tuning} & \textbf{Links} \\
\midrule
\endfirsthead

% == CHANGED HERE ==
% Added \rowcolor{white} to this row to remove striping
\rowcolor{white}
\multicolumn{8}{c}{\tablename\ \thetable\ -- Continued from previous page} \\
\toprule
% == CHANGED HERE ==
% Added a background color to the header row (for subsequent pages)
\rowcolor{white}
\textbf{Time} & \textbf{Method} & \textbf{Venue} & \textbf{Task(s)} & \textbf{Tool(s)} & \textbf{Agent Backbone} & \textbf{Tuning} & \textbf{Links} \\
\midrule
\endhead

% == CHANGED HERE ==
% Added \rowcolor{white} to this row to remove striping
\rowcolor{white}
\multicolumn{8}{r}{\textit{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot

% ==== Section 1 ====
% This \rowcolor will now correctly reset the \rowcolors* counter
\rowcolor{sectionblue}\multicolumn{8}{c}{\textbf{SFT \& Off-Policy Methods}} \\
\midrule
2024.10 & LeReT & ICLR'25 & IR & Dense Retriever & LLaMA3, Gemma2 & DPO-like (IPO) & \href{https://arxiv.org/abs/2410.23214}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/sher222/LeReT}{\faGithub} \\
2024.10 & ToolFlow & NAACL'25 & Tool-Calling &  APIs & LLaMA3.1 & SFT & \href{https://arxiv.org/abs/2410.18447}{\textcolor{cardinal}{\faFilePdf}} \\
% 2024.10 & LeanAgent & ICLR’25 & Formal Theorem Proving & LeanDojo & ByT5 (ReProver) & SFT & \href{https://arxiv.org/abs/2410.06209}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/lean-dojo/LeanAgent}{\faGithub} \\
2024.06 & TP-LLaMA & NeurIPS'24 & Tool-Calling &  APIs & LLaMA2 & SFT, DPO & \href{https://arxiv.org/abs/2406.07115}{\textcolor{cardinal}{\faFilePdf}} \\
2024.05 & AutoTools & WWW'25 & Tool-Calling &  APIs & GPT4, LLaMA3, Mistral & SFT & \href{https://arxiv.org/abs/2405.16533}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/mangopy/AutoTools}{\faGithub} \\
2024.03 & CYCLE &OOPSLA'24& Coding &Code Executor &CodeGen, StarCoder &SFT& \href{https://arxiv.org/abs/2403.18746}{\textcolor{cardinal}{\faFilePdf}} \\
2024.02 & RetPO & NAACL'25 & IR & Retriever & LLaMA2-7B& SFT, DPO & \href{https://arxiv.org/abs/2402.11827}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/dmis-lab/RetPO}{\faGithub}\\
2024.02 & CodeAct & ICML'24 & Coding & Code Executor & LLaMA2, Mistral & SFT & \href{https://arxiv.org/abs/2402.01030}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/xingyaoww/code-act}{\faGithub} \\
2024.01 & NExT & ICML'24 & Program Repair & Code Executor & PaLM2 & SFT & \href{https://arxiv.org/abs/2404.14662}{\textcolor{cardinal}{\faFilePdf}} \\
2023.07 & ToolLLM & ICLR'24 & Tool-Calling, API Planning, Multi-Tool Reasoning & Real-World APIs & LLaMA, Vicuna & SFT & \href{https://arxiv.org/abs/2307.16789}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/OpenBMB/ToolBench}{\faGithub} \\
2023.06 & ToolAlpaca & arXiv & Multi-Turn Tool-Use & Simulated APIs & Vicuna & SFT & \href{https://arxiv.org/abs/2306.05301}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/tangqiaoyu/ToolAlpaca}{\faGithub} \\
2023.05 & Gorilla & NeurIPS'24 & Tool-Calling, API Retrieval &  APIs & LLaMA & SFT & \href{https://arxiv.org/abs/2305.15334}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/ShishirPatil/gorilla}{\faGithub} \\
2023.05 & TRICE & NAACL'24 & Math Reasoning, QA & Calculator, WikiSearch, Atlas QA Model, NLLB Translator & ChatGLM, Alpaca, Vicuna & SFT, Contrastive Learning & \href{https://arxiv.org/abs/2305.13068}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/zjunlp/TRICE}{\faGithub} \\
2023.02 & Toolformer & NeurIPS'23 & QA, Math & Calculator, QA system, Search Engine, Translation System, Calendar & GPT-J & SFT & \href{https://arxiv.org/abs/2302.04761}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/conceptofmind/toolformer}{\faGithub} \\
\midrule
% ==== Section 2 ====
% This \rowcolor will also reset the counter, so striping is consistent
\rowcolor{sectiongreen}\multicolumn{8}{c}{\textbf{RLVR Methods}} \\
\midrule
2025.11 & Orion & arXiv & IR & Retrievers & LFM2 & GRPO & \href{https://arxiv.org/abs/2511.07581}{\textcolor{cardinal}{\faFilePdf}}\\
2025.10 & olmOCR2 & arXiv & Document OCR & Synthetic Document Verifier & Qwen2.5-VL & SFT, GRPO & \href{https://arxiv.org/abs/2510.19817}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/allenai/olmocr}{\faGithub} \\
2025.10 & AlphaProof & Nature & Formal Theorem Proving  & Lean Solver & Transformer (3B Enc-Dec) & SFT, AlphaZero, TTRL & \href{https://www.nature.com/articles/s41586-025-09833-y}{\textcolor{cardinal}{\faFilePdf}}\\
2025.10 & ToolExpander & arXiv & Tool-Calling &  Tool APIs & Qwen2.5 & SFT, GRPO & \href{https://arxiv.org/abs/2510.07737}{\textcolor{cardinal}{\faFilePdf}} \\
2025.09 & WebGen-Agent & arXiv & Website Generation & VLM, GUI Agent, Code Executor & Qwen2.5-Code, Qwen3 & SFT, Step-GRPO & \href{https://arxiv.org/abs/2509.22644}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/mnluzimu/WebGen-Agent}{\faGithub} \\
2025.09 & Tool-R1 & arXiv & Tool-Augmented Reasoning, QA & Code Execution, Multimedia Tools & Qwen2.5 & GRPO & \href{https://arxiv.org/abs/2509.12867}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/YBYBZhang/Tool-R1}{\faGithub} \\
2025.08 & FTRL & arXiv & Multi-Step Tool-Use & Simulated APIs & Qwen3 & GRPO & \href{https://arxiv.org/abs/2508.08791}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/bytedance/FTRL}{\faGithub} \\
2025.08 & Goedel-Prover-V2 & arXiv & Formal Theorem Proving & Lean Compiler & Qwen3 & SFT, GRPO & \href{https://arxiv.org/abs/2508.03613}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/Goedel-LM/Goedel-Prover-V2}{\faGithub} \\
2025.06 & Router-R1 & NeurIPS'25 & Multi-Round Routing & LLM Routing Pool & Qwen2.5, LLaMA3.2 & PPO & \href{https://arxiv.org/abs/2506.09033}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/ulab-uiuc/Router-R1}{\faGithub} \\
2025.05 & R1-Code-Interpreter & arXiv & Coding & Code Execution Sandbox & Qwen2.5 & GRPO & \href{https://arxiv.org/abs/2505.21668}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/yongchao98/R1-Code-Interpreter}{\faGithub} \\
2025.05 & Tool-N1 & arXiv & Tool-Calling & Tool APIs & Qwen2.5 & GRPO & \href{https://arxiv.org/abs/2505.00024}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/NVlabs/Tool-N1}{\faGithub} \\
2025.04 & SQL-R1 & NeurIPS'25 & Text2SQL Search & SQL Engine & Qwen2.5, OmniSQL & SFT, GRPO & \href{https://arxiv.org/abs/2504.08600}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/DataArcTech/SQL-R1}{\faGithub} \\
2025.03 & Rec-R1 & TMLR'25 & Recommendation Optimization & Recommendation System & Qwen2.5, LLaMA3.2 & GRPO & \href{https://openreview.net/forum?id=YBRU9MV2vE}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/linjc16/Rec-R1}{\faGithub} \\
2025.03 & ReZero & arXiv & Web Search, IR & Web Search Engine & LLaMA3.2 & GRPO & \href{https://arxiv.org/abs/2504.11001}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/janhq/ReZero}{\faGithub} \\
2025.03 & Code-R1 & --- & Coding & Code Executor & Qwen2.5 & GRPO & \href{https://github.com/ganler/code-r1}{\faGithub} \\
2025.02 & DeepRetrieval & COLM'25 & Web Search, IR, Text2SQL & Search Engine, Retrievers, SQL exec. & Qwen2.5, LLaMA3.2 & PPO, GRPO & \href{https://arxiv.org/abs/2503.00223}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/pat-jj/DeepRetrieval}{\faGithub} \\
2025.01 & DeepSeek-R1-Zero (Code) & Nature & Coding & Code Executor & DeepSeek-V3-Base & GRPO & \href{https://arxiv.org/abs/2501.12948}{\textcolor{cardinal}{\faFilePdf}}  \\
% 2024.10 & InternLM2.5-StepProver & arXiv & Formal Theorem
% Proving & Lean 4 & InternLM2.5 & SFT & \href{https://arxiv.org/abs/2410.15700} {\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/InternLM/InternLM-Math}{\faGithub}  \\
2024.10 & RLEF & ICML'25 & Coding & Code Executor & LLaMA3.1 & PPO & \href{https://arxiv.org/abs/2410.02089}{\textcolor{cardinal}{\faFilePdf}} \\
2024.08 & DeepSeek-Prover-V1.5 & ICLR’25 & Formal Theorem Proving & Lean 4 Prover & DeepSeek-Prover-V1.5-RL & SFT, GRPO & \href{https://arxiv.org/abs/2408.08152}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/deepseek-ai/DeepSeek-Prover-V1.5}{\faGithub} \\
2024.05 & LeDex & NeurIPS'24 & Coding & Code Executor & StarCoder \& CodeLlaMA & SFT, PPO & \href{https://arxiv.org/abs/2405.18649}{\textcolor{cardinal}{\faFilePdf}} \\

\end{longtable}
\normalsize

==> tables/a2_methods.tex <==
% --- Your original color definitions ---
\definecolor{sectionblue}{RGB}{230,245,255}
\definecolor{sectiongreen}{RGB}{235,255,235}
\definecolor{cardinal}{RGB}{180,0,0}

% --- NEW: Color for the table header ---
\definecolor{white}{RGB}{255,255,255}

% Stylish longtable
\small
%
% == CHANGED HERE ==
% Use \rowcolors* (with asterisk) to reset counter after manual \rowcolor
% Start at row 1, so the first data row after a section header is gray
%
\rowcolors*{1}{gray!7}{white}
\renewcommand{\arraystretch}{1.15}

\begin{longtable}[t]{>{\raggedright\arraybackslash}p{1.2cm}
                  >{\raggedright\arraybackslash}p{2.2cm}
                  >{\raggedright\arraybackslash}p{1.5cm}
                  >{\raggedright\arraybackslash}p{2.4cm}
                  >{\raggedright\arraybackslash}p{2.3cm}
                  >{\raggedright\arraybackslash}p{2.5cm}
                  >{\raggedright\arraybackslash}p{2.1cm}
                  >{\raggedright\arraybackslash}p{0.8cm}}
\rowcolor{white}
\caption{A2 Methods: Agent Output Signaled Agent Adaptation} \\

\toprule
% == CHANGED HERE ==
% Added a background color to the header row
\rowcolor{white}
\textbf{Time} & \textbf{Method} & \textbf{Venue} & \textbf{Task(s)} & \textbf{Tool(s)} & \textbf{Agent Backbone} & \textbf{Tuning} & \textbf{Links} \\
\midrule
\endfirsthead

% == CHANGED HERE ==
% Added \rowcolor{white} to this row to remove striping
\rowcolor{white}
\multicolumn{8}{c}{\tablename\ \thetable\ -- Continued from previous page} \\
\toprule
% == CHANGED HERE ==
% Added a background color to the header row (for subsequent pages)
\rowcolor{white}
\textbf{Time} & \textbf{Method} & \textbf{Venue} & \textbf{Task(s)} & \textbf{Tool(s)} & \textbf{Agent Backbone} & \textbf{Tuning} & \textbf{Links} \\
\midrule
\endhead

% == CHANGED HERE ==
% Added \rowcolor{white} to this row to remove striping
\rowcolor{white}
\multicolumn{8}{r}{\textit{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot
\rowcolor{red!5}\multicolumn{8}{c}{\textbf{w/o Tools}} \\
\midrule
2025.10 & Empower & arXiv & Coding & --- & Gemma3 & SFT & \href{https://arxiv.org/abs/2510.13709}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/festusev/codegen_empowerment/tree/main}{\faGithub} \\ 
2025.10 & KnowRL & arXiv & Knowledge Calibration & --- &LLaMA3.1, Qwen2.5 & REINFORCE++ & 
\href{https://arxiv.org/abs/2510.11407}{\textcolor{cardinal}{\faFilePdf}} \href{https://anonymous.4open.science/r/KnowRL-5BF0}{\faGithub} \\ 
2025.10 & GRACE & arXiv & Embedding Tasks & --- & Qwen2.5, Qwen3, LLaMA3.2 & GRPO & \href{https://arxiv.org/abs/2510.04506}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/GasolSun36/GRACE}{\faGithub} \\ 
2025.06 & Magistral & arXiv & Math, Coding & --- & Magistral & PPO, GRPO & \href{https://arxiv.org/abs/2506.10910}{\textcolor{cardinal}{\faFilePdf}} \\ 
2025.05 & metaTextGrad & NeurIPS'25 & QA, Math, Word Sorting & --- & Qwen3-235B-A22B, Claude-3.5-Sonnet & Prompt Engineering & \href{https://arxiv.org/abs/2505.18524}{\textcolor{cardinal}{\faFilePdf}}  \href{https://github.com/zou-group/metatextgrad}{\faGithub} \\ 
2025.05 & EHRMind & arXiv & EHR-based Reasoning & --- &  LLaMA3 & SFT, GRPO & \href{https://arxiv.org/abs/2505.24105}{\textcolor{cardinal}{\faFilePdf}}  \\ 
2025.01 & Kimi k1.5 & arXiv & Math, Coding & --- & Kimi k1.5 & GRPO & \href{https://arxiv.org/abs/2501.12948}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/MoonshotAI/Kimi-k1.5}{\faGithub} \\ 
2025.01 & DeepSeek-R1-Zero (Math) & Nature & Math & --- & DeepSeek-V3 & GRPO & \href{https://arxiv.org/abs/2501.12948}{\textcolor{cardinal}{\faFilePdf}}  \\ 
2024.09 & SCoRe & ICLR'25 &Math, Coding, QA &--- & Gemini1.0 Pro, Gemini1.5 Flash & REINFORCE &\href{https://arxiv.org/abs/2409.12917}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/BY571/SCoRe}{\faGithub} \\
2024.07 & RISE &NeurIPS'24& Math &---&LLaMA2, LLaMA3, Mistral&SFT& \href{https://arxiv.org/abs/2407.18219}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/cmu-mind/RISE}{\faGithub} \\
2024.06 & TextGrad & Nature& Code Optimization, Molecule Optimization, etc. & --- & GPT3.5, GPT4o & Prompt Engineering & \href{https://arxiv.org/abs/2406.07496}{\textcolor{cardinal}{\faFilePdf}}  \href{https://github.com/zou-group/textgrad}{\faGithub} \\ 
2023.03 & Self-Refine & NeurIPS'23 &Dialogue, Math, Coding &--- & GPT3.5, GPT4, CODEX & Prompt Engineering &\href{https://arxiv.org/abs/2303.17651}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/madaan/self-refine}{\faGithub} \\ 
\midrule
\rowcolor{orange!5}\multicolumn{8}{c}{\textbf{w/ Tools}} \\
\midrule
2025.10 & TT-SI & arXiv & Tool Calling &Tool APIs& Qwen2.5 & Test-Time Fine-Tuning  & \href{https://arxiv.org/abs/2510.07841}{\textcolor{cardinal}{\faFilePdf}}  \\
2025.10 & A$^2$FM & arXiv & Web Navigation, Math, QA &Search Engine, Crawl, Code Executor& Qwen2.5 & APO,GRPO & \href{https://arxiv.org/abs/2510.12838}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/OPPO-PersonalAI/Adaptive_Agent_Foundation_Models}{\faGithub}  \\
2025.09 & VerlTool & arXiv & Math, QA, SQL, Visual, Web Search, Coding & Code Interpreter, Search Engine, SQL Executor, Vision Tools & Qwen2.5, Qwen3 & GRPO & \href{https://arxiv.org/abs/2509.01055}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/TIGER-AI-Lab/verl-tool}{\faGithub} \\ 
2025.08 & MedResearcher-R1 & arXiv & Medical QA &Medical Retriever, Web Search API, Document Reader& MedResearcher-R1&SFT, GRPO& \href{https://arxiv.org/abs/2508.14880}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/AQ-MedAI/MedResearcher-R1}{\faGithub}  \\
2025.08 & Agent Lightning & arXiv & Text2SQL, Math &SQL Executor, Retriever, Calculator& LLaMA3.2 & LightningRL & \href{https://arxiv.org/abs/2508.03680}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/microsoft/agent-lightning}{\faGithub}  \\
2025.07 & CodePRM & ACL'25 &Coding &Code Executor & Qwen2.5-Coder   & SFT &\href{https://aclanthology.org/2025.findings-acl.428/}{\textcolor{cardinal}{\faFilePdf}} \\
2025.07 & DynaSearcher & arXiv & QA &Document Search, KG Search& Qwen2.5, LLaMA3.1&GRPO& \href{https://arxiv.org/abs/2507.17365}{\textcolor{cardinal}{\faFilePdf}} \href{https://modelscope.cn/home}{\faGithub}  \\
2025.06 & MMSearch-R1 & arXiv & QA, VQA &Image Search, Web Browser, Retriever& Qwen2.5&REINFORCE, SFT& \href{https://arxiv.org/abs/2506.20670}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/EvolvingLMMs-Lab/multimodal-search-r1}{\faGithub}  \\
2025.06 & Self-Challenging & arXiv &Multi-Turn Function-Calling, Calculation &Code Interpreter, Web Browser & LLaMA3.1   & REINFORCE, SFT &\href{https://arxiv.org/abs/2506.01716}{\textcolor{cardinal}{\faFilePdf}} \\
2025.05 & StepSearch & EMNLP'25 & QA &Search Engine, Retriever& Qwen2.5&StePPO& \href{https://arxiv.org/abs/2505.15107}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/Zillwang/StepSearch}{\faGithub}  \\
2025.05 & ZeroSearch & arXiv & QA &Search Engine, Web Search& Qwen2.5, LLaMA3.2&REINFORCE, GPRO, PPO, SFT& \href{https://arxiv.org/abs/2505.04588}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/Alibaba-NLP/ZeroSearch}{\faGithub}  \\
2025.05 & AutoRefine & NeurIPS'25 & QA &Retriever& Qwen2.5&GRPO& \href{https://arxiv.org/abs/2505.11277}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/syr-cn/AutoRefine}{\faGithub}  \\
2025.04 & ReTool & arXiv & Math &Code  Interpreter& Qwen2.5 &PPO& \href{https://arxiv.org/abs/2504.11536}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/ReTool-RL/ReTool}{\faGithub}  \\
2025.04 & ToolRL & arXiv & Tool Calling & Tool APIs& Various Models&GRPO& \href{https://arxiv.org/abs/2504.13958}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/qiancheng0/ToolRL}{\faGithub}  \\
2025.04 & DeepResearcher & arXiv & QA, Reasoning, Deep Research &Web Search API, Web Browser& Qwen2.5&GRPO& \href{https://arxiv.org/abs/2504.03160}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/GAIR-NLP/DeepResearcher}{\faGithub}  \\
2025.03 & ReSearch & NeurIPS'25 & QA &Search Engine, Retriever& Qwen2.5 &GRPO& \href{https://arxiv.org/abs/2503.19470}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/Agent-RL/ReCall}{\faGithub}  \\
2025.03 & Search-R1 & COLM'25 & QA &Search Engine, Retriever& Qwen2.5 &PPO, GRPO& \href{https://arxiv.org/abs/2503.09516}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/PeterGriffinJin/Search-R1}{\faGithub}  \\
2025.03 & R1-Searcher & arXiv & QA &Retriever& LLaMA3.1, Qwen2.5&REINFORCE++& \href{https://arxiv.org/abs/2503.05592}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/RUCAIBox/R1-Searcher}{\faGithub}  \\
2025.02 & RAS & arXiv & QA & Retriever& LLaMA2, LLaMA3.2 &SFT& \href{https://arxiv.org/abs/2502.10996}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/pat-jj/RAS}{\faGithub}  \\
2025.01 & Agent-R & arXiv & Various Tasks &Monte Carlo Tree Search& Qwen2.5, LLaMA3.2&SFT& \href{https://arxiv.org/abs/2501.11425}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/ByteDance-Seed/Agent-R}{\faGithub}  \\
2024.06 & Re-ReST &EMNLP'24& QA, VQA, Sequential Decision, Coding &Tool APIs&Various Models&DPO& \href{https://arxiv.org/abs/2406.01495}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/PlusLabNLP/Re-ReST}{\faGithub} \\
2024.06 & RPG &EMNLP'24& QA, Reasoning&Search Engine, Retriever &LLaMA2, GPT3.5&SFT& \href{https://arxiv.org/abs/2406.14979}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/haruhi-sudo/RPG}{\faGithub} \\
2023.10 & Self-RAG &ICLR'24& QA, Fact Verification &Retriever&LLaMA2&SFT& \href{https://arxiv.org/abs/2310.11511}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/AkariAsai/self-rag}{\faGithub} \\
2023.10 & FireAct & arXiv & QA &Search API& GPT3.5, LLaMA2, CodeLLaMA &SFT& \href{https://arxiv.org/abs/2310.05915}{\textcolor{cardinal}{\faFilePdf}} \href{https://fireact-agent.github.io}{\faGithub}  \\

\end{longtable}
\normalsize

==> tables/notation.tex <==
\begin{table}[h]
\centering
\caption{Summary of key notations used throughout the paper.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\toprule
\textbf{Notation} & \textbf{Description} \\
\midrule
$\mathcal{A}$ & Agent, a (main reasoning) foundation model parameterized by its internal configuration (e.g., prompt templates or model weights). \\
$\mathcal{T}$ & Tool, any external callable component that operates independently from the agent’s internal parameters. \\
$\mathcal{E}$ & External environment in which the agent or tool interacts and receives feedback. \\
$\mathcal{D}$ & Offline data, as alignment reference for agent or tool. \\
$\mathcal{O}(\cdot)$ & Objective function optimized during adaptation. \\
% $\pi$ & Policy function governing the agent’s behavior. \\
% $s, a, r$ & State, action, and reward in the agent–environment interaction. \\
\bottomrule
\end{tabular}}
\label{tab:notation}
\end{table}


==> tables/t2_methods.tex <==
% --- Your original color definitions ---
\definecolor{sectionblue}{RGB}{230,245,255}
\definecolor{sectiongreen}{RGB}{235,255,235}
\definecolor{cardinal}{RGB}{180,0,0}

% --- NEW: Color for the table header ---
\definecolor{white}{RGB}{255,255,255}

% Stylish longtable
\small
%
% == CHANGED HERE ==
% Use \rowcolors* (with asterisk) to reset counter after manual \rowcolor
% Start at row 1, so the first data row after a section header is gray
%
\rowcolors*{1}{gray!7}{white}
\renewcommand{\arraystretch}{1.15}

\begin{longtable}{>{\raggedright\arraybackslash}p{1.2cm}
                  >{\raggedright\arraybackslash}p{2.0cm}
                  >{\raggedright\arraybackslash}p{1.5cm}
                  >{\raggedright\arraybackslash}p{2.4cm}
                  >{\raggedright\arraybackslash}p{2.5cm}
                  >{\raggedright\arraybackslash}p{2.5cm}
                  >{\raggedright\arraybackslash}p{2.1cm}
                  >{\raggedright\arraybackslash}p{0.8cm}}
\rowcolor{white}
\caption{T2 Methods: Tool Adaptation w/ Agent Supervision} \\

\toprule
% == CHANGED HERE ==
% Added a background color to the header row
\rowcolor{white}
\textbf{Time} & \textbf{Method} & \textbf{Venue} & \textbf{Task(s)} & \textbf{Tool Backbone} & \textbf{Agent Backbone} & \textbf{Tuning} & \textbf{Links} \\
\midrule
\endfirsthead

% == CHANGED HERE ==
% Added \rowcolor{white} to this row to remove striping
\rowcolor{white}
\multicolumn{8}{c}{\tablename\ \thetable\ -- Continued from previous page} \\
\toprule
% == CHANGED HERE ==
% Added a background color to the header row (for subsequent pages)
\rowcolor{white}
\textbf{Time} & \textbf{Method} & \textbf{Venue} & \textbf{Task(s)} & \textbf{Tool Backbone} & \textbf{Agent Backbone} & \textbf{Tuning} & \textbf{Links} \\

\midrule
\endhead

% == CHANGED HERE ==
% Added \rowcolor{white} to this row to remove striping
\rowcolor{white}
\multicolumn{8}{r}{\textit{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot
\rowcolor{sectionblue}\multicolumn{8}{c}{\textbf{Earlier Methods}} \\
\midrule
2025.06 & Sysformer & arXiv & QA & Small Transformer  &  LLaMA-2-7B, LLaMA-3.1-8B, Mistral-7B, Phi-3.5-mini, Zephyr-7B-beta &Supervised Learning & \href{https://arxiv.org/abs/2506.15751}{\textcolor{cardinal}{\faFilePdf}} \\

2024.10 & Matryoshka Pilot & NeurIPS'25 & Math, Planning, Reasoning & LLaMA3-8B, Qwen2.5-7B  &  GPT-4o-Mini, GPT-3.5-Turbo &DPO, IDPO & \href{https://arxiv.org/abs/2410.20749}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/lichangh20/Matryoshka}{\faGithub}\\

2024.06 & CoBB & EMNLP'24 & QA, Math & Mistral-7b-inst-v2  &  GPT-3.5-Turbo, Claude-3-Haiku, Phi-3-mini-4k-inst, Gemma-1.1-7B-it, Mistral-7B-inst-v2 &SFT, ORPO & \href{https://arxiv.org/abs/2406.18695}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/bbuing9/CoBB}{\faGithub}\\

2024.05 & Medadapter & EMNLP'24 & Medical QA, NLI, RQE & BERT-Base-Uncased  &  GPT-3.5-Turbo &SFT, BPO & \href{https://arxiv.org/abs/2405.03000}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/wshi83/MedAdapter}{\faGithub}\\

2024.03 & BLADE & AAAI'25 & QA &  BLOOMZ-1b7 &  ChatGPT, ChatGLM, Baichuan, Qwen &SFT, BPO & \href{https://arxiv.org/abs/2403.18365}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/CSHaitao/BLADE}{\faGithub}\\

2024.02 & ARL2 & ACL'24 & QA & LLaMA2-7B  &  GPT-3.5-Turbo &Contrastive Learning & \href{https://arxiv.org/abs/2402.13542}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/zhanglingxi-cs/ARL2}{\faGithub}\\

2024.02 & EVOR & EMNLP'24 &  Coding & GPT-3.5-Turbo &  GPT-3.5-Turbo, CodeLLaMA &Prompt Engineering & \href{https://arxiv.org/abs/2402.12317}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/xlang-ai/EVOR}{\faGithub}\\

2024.02 & Bbox-Adapter & ICML'24 & QA & DeBERTa-v3-base (0.1B), DeBERTa-v3-large (0.3B) &  GPT-3.5-Turbo, Mixtral-8x7B &Contrastive Learning & \href{https://arxiv.org/abs/2402.08219}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/haotiansun14/BBox-Adapter}{\faGithub}\\

2024.01 & Proxy-Tuning & COLM'24 & QA, Math, Code & LLaMA2-7B & LLaMA2-70B & Proxy-Tuning & \href{https://arxiv.org/abs/2401.08565}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/alisawuffles/proxy-tuning}{\faGithub}\\

2024.01 & BGM & ACL'24  & QA & T5-XXL-11B  & PaLM2-S  & SFT, PPO & \href{https://arxiv.org/abs/2401.06954}{\textcolor{cardinal}{\faFilePdf}} \\

2023.10 & RA-DIT & ICLR'24  & Knowledge-Intensive Tasks (MMLU, NQ, TQA, ELI5, HotpotQA, etc.) & DRAGON+  & LLaMA-65B & SFT, LSR & \href{https://arxiv.org/abs/2310.01352}{\textcolor{cardinal}{\faFilePdf}} \\

2023.06 & LLM-R & EACL'24  &  Zero-shot NLU (QA, NLI, Paraphrase, etc.) & E5-base  & GPT-Neo-2.7B, LLaMA-13B, GPT-3.5-Turbo & Contrastive Learning & \href{https://arxiv.org/abs/2307.07164}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/microsoft/LMOps/tree/main/llm_retriever}{\faGithub}\\

2023.05 & AAR & ACL'23  & Zero-Shot Generalization (MMLU, PopQA) & ANCE, Contriever  & Flan-T5-Small, InstructGPT & Contrastive Learning & \href{https://arxiv.org/abs/2305.17331}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/OpenMatch/Augmentation-Adapted-Retriever}{\faGithub}\\

2023.05 & ToolkenGPT &	NeurIPS'23 &Numerical Reasoning, QA, Plan Generation & Token Embedding &GPT-J 6B, OPT-6.7B, OPT-13B & Proxy-Tuning & \href{https://arxiv.org/abs/2305.11554}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/Ber666/ToolkenGPT}{\faGithub}\\

2023.03 & UPRISE  & EMNLP'23 & Zero-shot NLU (QA, NLI, etc.) &GPT-Neo-2.7B &BLOOM-7.1B, OPT-66B, GPT-3-175B& Contrastive Learning& \href{https://aclanthology.org/2023.emnlp-main.758/}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/microsoft/LMOps}{\faGithub}\\

2023.01 & REPLUG & NAACL'24 & QA & Contriever & GPT3-175B, PaLM, Codex, LLaMA-13B   &  Proxy-Tuning, LSR & \href{https://aclanthology.org/2024.naacl-long.463.pdf}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/swj0419/REPLUG}{\faGithub} \\
\midrule
\rowcolor{sectiongreen}\multicolumn{8}{c}{\textbf{RLVR Methods}} \\
\midrule
2025.10 & AgentFlow & arXiv &  Web Search, Planning, Reasoning, Math & Qwen2.5-7B & Qwen2.5-7B  &  Flow-GRPO & \href{https://arxiv.org/abs/2510.05592}{\textcolor{cardinal}{\faFilePdf}}
\href{https://github.com/lupantech/AgentFlow}{\faGithub} \\

2025.10 & QAgent& arXiv &  QA & Qwen2.5-3B & Qwen-7B &  GRPO & \href{https://arxiv.org/abs/2510.08383}{\textcolor{cardinal}{\faFilePdf}}
\href{https://github.com/LivingFutureLab/QAgent}{\faGithub} \\

2025.10 & Advisor Models& arXiv &  Math, Reasoning & Qwen2.5-7B, Qwen3-8B & GPT-4o-Mini, GPT-5, Claude4-Sonnet, GPT-4.1-Mini  &  GRPO & \href{https://arxiv.org/abs/2510.02453}{\textcolor{cardinal}{\faFilePdf}}
\href{https://github.com/az1326/advisor-models}{\faGithub} \\

2025.10	& AutoGraph-R1	&arXiv	&KG Construction &KG Constructor (Qwen2.5-3B/7B)	&Frozen RAG Generator (Qwen2.5-7B)	&GRPO  & \href{https://arxiv.org/abs/2510.15339}{\textcolor{cardinal}{\faFilePdf}}
\href{https://github.com/HKUST-KnowComp/AutoGraph-R1}{\faGithub}\\

2025.10 & MAE & arXiv &  Math, Coding, QA & Qwen2.5-3B & Qwen2.5-3B  &  REINFORCE++ & \href{https://arxiv.org/abs/2510.23595}{\textcolor{cardinal}{\faFilePdf}}
\href{https://github.com/ulab-uiuc/Multi-agent-Evolve}{\faGithub} \\

2025.09 & Mem-$\alpha$ & arXiv &  Test-Time Learning, Long-Range Understanding & Qwen3-4B & Qwen3-4B, Qwen3-32B, GPT-4.1-Mini  &  GRPO & \href{https://arxiv.org/abs/2509.25911}{\textcolor{cardinal}{\faFilePdf}}
\href{https://github.com/wangyu-ustc/Mem-alpha}{\faGithub} \\

2025.08 & AI-SearchPlanner & arXiv & QA & Qwen3-32B & Qwen2.5-7B &  PPO & \href{https://arxiv.org/abs/2508.20368}{\textcolor{cardinal}{\faFilePdf}} \\

2025.08 & Memento & arXiv & Long-Horizon Reasoning, Web Research, QA, Academic Reasoning & Q-function (two-layer MLPs) & GPT-4.1  &  Soft Q-Learning & \href{https://arxiv.org/abs/2508.16153}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/Agent-on-the-Fly/Memento}{\faGithub}\\

2025.08 & R-Zero & arXiv & Math, Reasoning & Qwen3-4B, Qwen3-8B, OctoThinker-3B, OctoThinker-8B  &  Qwen3-4B, Qwen3-8B, OctoThinker-3B, OctoThinker-8B &GRPO & \href{https://arxiv.org/abs/2508.05004}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/Chengsong-Huang/R-Zero}{\faGithub}\\

2025.05 & s3 & EMNLP'25 & QA & Qwen2.5-7B  &  Qwen2.5-7B, Qwen2.5-14B, Claude-3-Haiku &PPO & \href{https://arxiv.org/abs/2505.14146}{\textcolor{cardinal}{\faFilePdf}} \href{https://github.com/pat-jj/s3}{\faGithub}\\

\end{longtable}
\normalsize
